Proof of Church's Thesis

We prove that if our calculating capability is that of a universal Turing machine with a finite tape, then Church's thesis is true. This way we accomplish Post (1936) program.

==> fonts.tex <==
% FONTS.TEX (RMCG19940923)

\catcode`\@=11

% Adaptado de pdcfsel.tex (v 3.5, 1995/03/28) by P. Damian Cugley

\def\expcs#1#2{\expandafter#1\csname#2\endcsname}
\def\noexpcs{\expcs\noexpand}

\def\loadfont#1#2{\ifx#1\relax \FSELloadfont#1{#2}\else
 \ifx#1\UNDEFINED \FSELloadfont#1{#2}\fi\fi}

\def\FSELloadfont#1#2{\edef#1{\global\font\noexpand#1#2\relax\noexpand#1}}

\def\xfontset#1#2#3{
    \def\f##1##2{\expcs\loadfont{#1##1}{##2#3}}
    \let\m=\f \let\M=\f
    \def\@##1##2##3{\expcs\loadfont{#1##2}{##3 at #3pt }}
    #2 }

\def\fontset#1#2#3#4#5#6{\xfontset{#1}{#2}{#3}%
    \expcs\edef{#1fonts}{%
       \noexpcs{#1mathsfonts}%
       \noexpand\FSELnicknames{#1}{#5}{#6}\noexpand#2%
       \noexpand\setbaselineskip{#4}%
       \noexpand\rm }%
       \expcs\def{#1mathsfonts}{\FSELloadmaths{#1}{#5}{#6}#2}}

\def\FSELnicknames#1#2#3{\let\@\relax
    \def\f##1##2{\expcs\edef{##1}{\noexpcs{#1##1}}}%
    \def\m##1##2{%
       \expcs\textfont{##1fam}\csname#1##1\endcsname
       \expcs\scriptfont{##1fam}\csname#2##1\endcsname
       \expcs\edef{##1}{%
           \fam\expcs\noexpand{##1fam}%
           \expcs\noexpand{#1##1}}}%
    \def\M##1{\expcs\scriptscriptfont{##1fam}\csname#3##1\endcsname
       \m{##1}}}

\def\setbaselineskip#1{\ifdim #1=\baselineskip \else
    \baselineskip#1\relax \normalbaselineskip\baselineskip
    \jot0.25\baselineskip
    \smallskipamount 0.25\baselineskip plus 0.083\baselineskip
       minus 0.083\baselineskip
    \medskipamount 0.5\baselineskip plus 0.167\baselineskip
       minus 0.167\baselineskip
    \bigskipamount 1\baselineskip plus 0.333\baselineskip
       minus 0.333\baselineskip
    \setbox\strutbox=\hbox{\vrule height 0.708\baselineskip
       depth 0.292\baselineskip width\z@}%
    \def\big##1{{\hbox{$\left##1\vbox to0.708\baselineskip
       {}\right.\n@space$}}}%
    \def\Big##1{{\hbox{$\left##1\vbox to0.958\baselineskip
       {}\right.\n@space$}}}%
    \def\bigg##1{{\hbox{$\left##1\vbox to1.208\baselineskip
       {}\right.\n@space$}}}%
    \def\Bigg##1{{\hbox{$\left##1\vbox to1.458\baselineskip
       {}\right.\n@space$}}}%
    \topskip=0.833\baselineskip \splittopskip=\topskip
    \abovedisplayskip=1\baselineskip
       plus0.25\baselineskip minus0.75\baselineskip
    \abovedisplayshortskip=0pt plus0.25\baselineskip
    \belowdisplayskip=\abovedisplayskip
    \belowdisplayshortskip=0.583\baselineskip
       plus0.25\baselineskip minus0.333\baselineskip
 \fi}

\def\FSELloadmaths#1#2#3{%
    \let\@\relax \def\f##1##2{}%
    \def\m##1##2{\csname#1##1\endcsname \csname#2##1\endcsname}%
    \def\M##1{\csname#3##1\endcsname \m{##1}}%
    \global\expcs\let{#1mathsfonts}\relax}

\chardef\rmfam=0 \chardef\mifam=1 \chardef\syfam=2

% Databases

\def\cmtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\xfontset{cmscriptscript}\cmtemplate{5}
\xfontset{cmscript}\cmtemplate{7}
\fontset{cm}\cmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\def\cmbtemplate{%
   \M{rm}{cmbx}\f{it}{cmbxti}\M{bf}{cmr}\f{sc}{cmcsc}%
   \f{sl}{cmbxsl}\f{tt}{cmtt}\@\M{mi}{cmmib10}\@\M{sy}{cmbsy10}}
\xfontset{cmbscriptscript}\cmbtemplate{5}
\xfontset{cmbscript}\cmbtemplate{7}
\fontset{cmb}\cmbtemplate{10}{12pt}{cmbscript}{cmbscriptscript}

\def\viiitemplate{%
   \m{rm}{cmr}\f{it}{cmti}\m{bf}{cmbx}%
   \f{sl}{cmsl}\f{tt}{cmtt}\m{mi}{cmmi}\m{sy}{cmsy}}
\xfontset{viiiscript}\viiitemplate{6}
\fontset{viii}\viiitemplate{8}{10pt}{viiiscript}{viiiscript}

\def\xiitemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xiisc{cmcsc10 at 12pt }
\loadfont\xiisy{cmsy10 at 12pt }
\xfontset{xiiscriptscript}\xiitemplate{6}
\xfontset{xiiscript}\xiitemplate{9}
\fontset{xii}\xiitemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}

\def\xiibtemplate{%
   \M{rm}{cmbx}\@\m{it}{cmbxti10}\M{bf}{cmr}\@\f{sc}{cmssbx10}%
   \@\f{sl}{cmbxsl10}\f{tt}{cmtt}\@\M{mi}{cmmib10}\@\M{sy}{cmbsy10}}
\xfontset{xiibscriptscript}\xiibtemplate{6}
\xfontset{xiibscript}\xiibtemplate{9}
\fontset{xiib}\xiibtemplate{12}{14.4pt}{xiibscript}{xiibscriptscript}

\def\xivtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \m{sl}{cmsl}\m{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xivrm{cmr12 at 14.4pt }
\loadfont\xivit{cmti12 at 14.4pt }
\loadfont\xivbf{cmbx12 at 14.4pt }
\loadfont\xivsc{cmcsc10 at 14.4pt }
\loadfont\xivsl{cmsl12 at 14.4pt }
\loadfont\xivtt{cmtt12 at 14.4pt }
\loadfont\xivmi{cmmi12 at 14.4pt }
\loadfont\xivsy{cmsy10 at 14.4pt }
\xfontset{xivscriptscript}\xivtemplate{7}
\xfontset{xivscript}\xivtemplate{10}
\fontset{xiv}\xivtemplate{14.4}{17.28pt}{xivscript}{xivscriptscript}

\def\xivbtemplate{%
   \M{rm}{cmbx}\@\m{it}{cmbxti10}\M{bf}{cmr}\@\f{sc}{cmr12}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\M{mi}{cmmib10}\@\M{sy}{cmbsy10}}
\loadfont\xivbrm{cmbx12 at 14.4pt }
\loadfont\xivbbf{cmr12 at 14.4pt }
\xfontset{xivbscriptscript}\xivbtemplate{7}
\xfontset{xivbscript}\xivbtemplate{10}
\fontset{xivb}\xivbtemplate{14.4}{17.28pt}{xivbscript}{xivbscriptscript}

\def\xviitemplate{%
   \M{rm}{cmr}\@\m{it}{cmti12}\M{bf}{cmbx}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\M{mi}{cmmi}\@\M{sy}{cmsy10}}
\loadfont\xviirm{cmr17 at 17.28pt }
\loadfont\xviibf{cmbx12 at 17.28pt }
\loadfont\xviimi{cmmi12 at 17.28pt }
\xfontset{xviiscriptscript}\xviitemplate{8}
\xfontset{xviiscript}\xviitemplate{12}
\fontset{xvii}\xviitemplate{17.28}{20.736pt}{xviiscript}{xviiscriptscript}

\def\xviibtemplate{%
   \@\m{rm}{cmbx12}\@\m{it}{cmbxti10}\m{bf}{cmr}\@\f{sc}{cmr17}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\loadfont\xviibbf{cmr17 at 17.28pt }
\xfontset{xviibscript}\xviibtemplate{12}
\fontset{xviib}\xviibtemplate{17.28}{20.736pt}{xviibscript}{xviibscript}

\def\xxitemplate{%
   \@\M{rm}{cmr12}\@\m{it}{cmti12}\@\M{bf}{cmbx12}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\@\M{mi}{cmmi12}\@\M{sy}{cmsy10}}
\xfontset{xxiscriptscript}\xxitemplate{10}
\xfontset{xxiscript}\xxitemplate{14.28}
\fontset{xxi}\xxitemplate{20.736}{25pt}{xxiscript}{xxiscriptscript}

\def\lmtemplate{%
   \M{rm}{texnansi-lmr}\m{it}{texnansi-lmri}%
   \M{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\M{mi}{cmmi}\M{sy}{cmsy}}
\fontset{lm}\lmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\loadfont\lmxiisy{cmsy10 at 12pt }
\fontset{lmxii}\lmtemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}
\fontset{lmix}\lmtemplate{9}{11pt}{cmscript}{cmscriptscript}

\def\lmviiitemplate{%
   \m{rm}{texnansi-lmr}\f{it}{texnansi-lmri}%
   \m{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\m{mi}{cmmi}\m{sy}{cmsy}}
\fontset{lmviii}\lmviiitemplate{8}{10pt}{viiiscript}{viiiscript}

\loadfont\lmxiizero{texnansi-lmr17 at 21pt }
\loadfont\lmxiione{texnansi-lmbx12 at 17pt }
\loadfont\lmxiitwo{texnansi-lmbx12 at 14.4pt }
\loadfont\lmzero{texnansi-lmr17}
\loadfont\lmone{texnansi-lmbx12 at 14.4pt }
\loadfont\lmtwo{texnansi-lmbx12}
\def\lmtitles{\def\fontzero{\lmzero}%
 \def\fontone{\lmone}\def\fonttwo{\lmtwo}}
\def\lmxiititles{\def\fontzero{\lmxiizero}%
 \def\fontone{\lmxiione}\def\fonttwo{\lmxiitwo}}

\def\pstemplate{%
   \@\M{rm}{ptmr8r}\@\M{it}{ptmri8r}\@\M{bf}{ptmb8r}\@\f{sc}{ptmrc8t}%
   \@\M{mi}{ptmri8t}\@\M{tt}{pcrr8r}}
\xfontset{psxscriptscript}\pstemplate{5}
\xfontset{psxscript}\pstemplate{7}
\fontset{psx}\pstemplate{10}{12pt}{psxscript}{psxscriptscript}

\xfontset{psxiiscriptscript}\pstemplate{6}
\xfontset{psxiiscript}\pstemplate{9}
\fontset{psxii}\pstemplate{12}{14.4pt}{psxiiscript}{psxiiscriptscript}

\xfontset{psxivscriptscript}\pstemplate{7}
\xfontset{psxivscript}\pstemplate{11}
\fontset{psxiv}\pstemplate{14.4}{17.28pt}{psxivscript}{psxivscriptscript}

\xfontset{psxviiscriptscript}\pstemplate{9}
\xfontset{psxviiscript}\pstemplate{14}
\fontset{psxvii}\pstemplate{17}{21pt}{psxviiscript}{psxviiscriptscript}

\xfontset{psxxiscriptscript}\pstemplate{10}
\xfontset{psxxiscript}\pstemplate{14}
\fontset{psxxi}\pstemplate{21}{25pt}{psxxiscript}{psxxiscriptscript}

\def\zerotemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\M{sl}{cmsl}%
   \M{tt}{cmtt}}
\loadfont\zerobf{cmbx12 at 17.28pt }
\loadfont\zeroit{cmti12 at 17.28pt }
\loadfont\zerosl{cmsl12 at 17.28pt }
\loadfont\zerott{cmtt12 at 17.28pt }
\xfontset{zeroscriptscript}\zerotemplate{9}
\xfontset{zeroscript}\zerotemplate{12}
\fontset{zero}\zerotemplate{17}{20.4pt}{zeroscript}{zeroscriptscript}

\def\onetemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\m{sl}{cmsl}%
   \m{tt}{cmtt}}
\loadfont\onerm{cmr12 at 14.4pt }
\loadfont\onebf{cmbx12 at 14.4pt }
\loadfont\oneit{cmti12 at 14.4pt }
\loadfont\onesl{cmsl12 at 14.4pt }
\loadfont\onett{cmtt12 at 14.4pt }
\xfontset{onescriptscript}\onetemplate{7}
\xfontset{onescript}\onetemplate{10}
\fontset{one}\onetemplate{14.4}{17.28pt}{onescript}{onescriptscript}

% Fonts for titles

\def\cmtitles{%
 \def\fontzero{\xviifonts\rm}%
 \def\fontone{\xivbfonts\rm}%
 \def\fonttwo{\xiibfonts\rm}%
 \def\fontthree{\cmbfonts\rm}%
}
\def\viiititles{%
 \def\fontzero{\xivbfonts\rm}%
 \def\fontone{\xiibfonts\rm}%
 \def\fonttwo{\cmbfonts\rm}%
}
\def\xiititles{%
 \def\fontzero{\xxifonts\rm}%
 \def\fontone{\xviibfonts\rm}%
 \def\fonttwo{\xivbfonts\rm}%
 \def\fontthree{\xiibfonts\rm}%
}
\def\psxtitles{%
 \def\fontzero{\psxviifonts\rm}%
 \def\fontone{\psxivfonts\bf}%
 \def\fonttwo{\psxiifonts\bf}%
}
\def\psxiititles{%
 \def\fontzero{\psxxifonts\rm}%
 \def\fontone{\psxviifonts\bf}%
 \def\fonttwo{\psxivfonts\bf}%
}
\cmtitles

\catcode`\@=12

\endinput


==> indexes.tex <==
% indexes.tex (RMCG20200315)

\ifx\utfon\undefined \input utf \fi

\catcode`\@=11

\catcode`\^^02=12 \catcode`\^^03=12 \catcode`\^^04=12 \catcode`\^^05=12

% Check files auxiliar.aux, auxiliar.ind

\newread\infile

\newif\ifauxf
\openin\infile=auxiliar.aux
\ifeof\infile \auxffalse \else \auxftrue \fi
\closein\infile

\newif\ifindf
\openin\infile=auxiliar.ind
\ifeof\infile \indffalse \else \indftrue \fi
\closein\infile

% pdf

\ifx\pdfoutput\undefined \csname newcount\endcsname\pdfoutput \fi

% \color{Red} ... \endcolor

\def\cmykWhite{0 0 0 0} \def\cmykDarkWhite{0 0 0 .3}
\def\cmykGray{0 0 0 .5} \def\cmykDarkGray{0 0 0 .7}
\def\cmykBlack{0 0 0 1} \def\cmykDarkBlack{.4 .3 .3 1}
\def\cmykYellow{0 0 1 0} \def\cmykDarkYellow{0 0 1 .7}
\def\cmykMagenta{0 1 0 0} \def\cmykDarkMagenta{0 1 0 .7}
\def\cmykCyan{1 0 0 0} \def\cmykDarkCyan{1 0 0 .7}
\def\cmykRed{0 1 1 0} \def\cmykDarkRed{0 1 1 .7}
\def\cmykGreen{1 0 1 0} \def\cmykDarkGreen{1 0 1 .7}
\def\cmykBlue{1 1 0 0} \def\cmykDarkBlue{1 1 0 .7}

\newcount\col@rstack
\def\pdf@color#1{\pdfcolorstack\col@rstack push {\csname cmyk#1\endcsname k}}
 \def\pdf@darkcolor#1{\pdfcolorstack\col@rstack push {\csname cmykDark#1\endcsname k}}
 \def\pdf@endcolor{\pdfcolorstack\col@rstack pop}
 \def\pdf@black{\pdfcolorstack\col@rstack push {0 g}}
\def\dvips@color#1{\special{color push cmyk \csname cmyk#1\endcsname}}
 \def\dvips@darkcolor#1{\special{color push cmyk \csname cmykDark#1\endcsname}}
 \def\dvips@endcolor{\special{color pop}}
 \def\dvips@black{\special{color push gray 0}}
\def\dvipdf@color#1{\special{pdf: bc [\csname cmyk#1\endcsname]}}
 \def\dvipdf@darkcolor#1{\special{pdf: bc [\csname cmykDark#1\endcsname]}}
 \def\dvipdf@endcolor{\special{pdf: ec}}
 \def\dvipdf@black{\special{pdf: bc [0]}}

\def\pdf@background#1{\pdfliteral page {q \csname cmyk#1\endcsname k \csname cmyk#1\endcsname K
 -144 -144 m 864 -144 l 864 1080 l -144 1080 l b Q}}
\def\dvips@background#1{\special{background cmyk \csname cmyk#1\endcsname}}
\def\dvipdf@background#1{\special{pdf: bgc [\csname cmyk#1\endcsname]}}

\ifcase\pdfoutput
 \ifx\dvips\undefined
  \special{pdf: sc [0]}\let\colorblack=\dvipdf@black
  \def\colors{\let\color=\dvipdf@color\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
  \def\darkcolors{\let\color=\dvipdf@darkcolor\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
  \let\background=\dvipdf@background
 \else
  \special{color gray 0}\let\colorblack=\dvips@black
  \def\colors{\let\color=\dvips@color\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
  \def\darkcolors{\let\color=\dvips@darkcolor\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
  \let\background=\dvips@background
 \fi
\else
 \col@rstack=\pdfcolorstackinit page {0 g}\let\colorblack=\pdf@black
 \def\colors{\let\color=\pdf@color\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
 \def\darkcolors{\let\color=\pdf@darkcolor\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
 \let\background=\pdf@background
\fi

\def\nocolor{\def\color##1{\relax}\def\truecolor##1{\relax}\def\endcolor{\relax}}
\nocolor % default value, \darkcolors intermediate with \colors

% type of links

\def\numlink#1{num \number#1}
\def\namelink#1{name {(\number#1)}}
\ifx\xmpinclude\undefined \let\typelink=\numlink \else \let\typelink=\namelink \fi

% \goto{Text in red}{123}

{\catcode`\#=12 \xdef\hash{#}}

\def\pdf@goto#1#2{\leavevmode
 \pdfstartlink attr{/F 4 /Border [0 0 0]} goto \typelink{#2}%
 \color{Red}#1\endcolor\pdfendlink\relax}
\def\dvips@goto#1#2{\leavevmode
 \special{html:<a href=\string"\hash\typelink{#2}\string">}%
 \color{Red}#1\endcolor\special{html:</a>}\relax}
\def\dvipdf@goto#1#2{\leavevmode
 \special{pdf: bann << /Type /Annot /Subtype /Link /Border [0 0 0]
   /A << /S /GoTo /D (\typelink{#2}) >> >>}\color{Red}#1\endcolor
 \special{pdf: eann}\relax}
\def\nolinks@goto#1#2{\leavevmode
 \closeout-1\color{Red}#1\endcolor\closeout-1\relax}
%\closeout-1 is just a whatsit, i.e. an extension as pdf commands are

% \dest

\newcount\d@stno

\def\pdf@dest{\global\advance\d@stno1
 \ifvmode \pdfdest \typelink{\d@stno} fitbh\else
  \vbox to0pt{\vss\pdfdest \typelink{\d@stno} fitbh\kern1pc}\fi}
\def\dvips@dest{\global\advance\d@stno1
 \ifvmode \special{html:<a name=\string"\typelink{\d@stno}\string">}
          \special{html:</a>}\else
  \vbox to0pt{\vss\special{html:<a name=\string"\typelink{\d@stno}\string">}
                  \special{html:</a>}\kern1pc}\fi}
\def\dvipdf@dest{\global\advance\d@stno1
 \ifvmode
  \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\else
  \vbox to0pt{\vss
   \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\kern1pc}\fi}
\def\nolinks@dest{\global\advance\d@stno1
 \ifvmode \closeout-1\else \vbox to0pt{\vss\closeout-1\kern1pc}\fi}

\ifcase\pdfoutput
 %\def\pdfcode#1\pdfendcode{\relax\closeout-1\relax}
 \ifx\dvips\undefined
  \def\links{\let\goto=\dvipdf@goto\let\dest=\dvipdf@dest}
 \else
  \def\links{\let\goto=\dvips@goto\let\dest=\dvips@dest}
 \fi
\else
 %\let\pdfcode=\relax \let\pdfendcode=\relax
 \def\links{\let\goto=\pdf@goto\let\dest=\pdf@dest}
\fi

\def\nolinks{\let\goto=\nolinks@goto\let\dest=\noliks@dest}
\links % default value

% \footnote

\def\footnoteoptions{\everypar{}} % \eightpt, for example
% adapted from [363]; parameter #2 (the text) is read later
\def\footnote#1{\let\@sf\empty
  \ifhmode\edef\@sf{\spacefactor\the\spacefactor}\/\fi
  \global\advance\d@stno1 \goto{#1}{\number\d@stno}\global\advance\d@stno-1% RMCG
  \@sf\vfootnote{#1}}
\def\vfootnote#1{\insert\footins\bgroup
  \interlinepenalty\interfootnotelinepenalty
  \splittopskip\ht\strutbox % top baseline for broken footnotes
  \splitmaxdepth\dp\strutbox \floatingpenalty\@MM
  \leftskip\z@skip \rightskip\z@skip \spaceskip\z@skip \xspaceskip\z@skip
  \footnoteoptions \textindent{#1}\footstrut\dest\futurelet\next\fo@t} % RMCG

% \pdf@ut calculates the number of branches in \@utno

\newtoks\pdft@k \pdft@k{}
\def\pdft@toc#1{\global\pdft@k=\expandafter{\the\pdft@k#1}}
\newcount\@utno \newcount\@uts
\newcount\@utss \newcount\@utt
\def\c@rcdr#1#2,{\edef\car{#1}\edef\cdr{#2}\ifx\cdr\empty\edef\cdr{0}\fi}
\def\pdf@ut{\expandafter\c@rcdr\the\pdft@k,\@uts=\car
 \global\pdft@k=\expandafter{\cdr}\toks0=\expandafter{\cdr}%
 \@utno=0 \@utss=\car \advance\@utss1
 \loop \expandafter\c@rcdr\the\toks0,\@utt=\car\toks0=\expandafter{\cdr}%
  \ifnum\@uts<\@utt \ifnum\@utss=\@utt\advance\@utno1\fi \repeat}

% Indexing

\def\ref#1{??} \def\refsc#1{??} \def\refpg#1{??} \def\refx#1#2{??}
% \toc{level}{text} \pdftocline{text}{\d@stno}
\let\toc=\gobbletwo \let\pdftocline=\gobbletwo
% \lbl{mnemonic}{replacement} \ndx{text}{type}
\let\lbl=\gobbletwo \let\ndx=\gobbletwo

% \pdfout{level}{title}{secid}
\def\pdfoutA#1#2#3{#3 #2}
\def\pdfoutB#1#2#3{#2}
\let\pdfout=\pdfoutA

\catcode`\(=13 \catcode`\)=13
 \def({\string\(} \def){\string\)}
\catcode`\(=12 \catcode`\)=12

\def\pdf@outline#1#2#3#4#5{\pdfoutline goto \typelink{#3}
 count \number\@utno {\pdfout{#1}{#2}{#4}}}
\def\dvips@outline#1#2#3#4#5{\special{ps: [ /Title (\pdfout{#1}{#2}{#4})
 /Count \number\@utno\space /Page #5 /OUT pdfmark}}
\def\dvipdf@outline#1#2#3#4#5{\special{pdf: out #1 <<
 /Title (\pdfout{#1}{#2}{#4}) /Dest (\typelink{#3}) >>}}

\def\star{*}
\def\@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\star\else
 \ifx\4\empty \let\pdfout=\pdfoutB \else
 \ifx\4\lq \let\pdfout=\pdfoutB \else
 \ifx\4\rq \let\pdfout=\pdfoutB \else
 \ifx\4\lbrack\let\pdfout=\pdfoutB \else
 \ifx\4\rbrack\let\pdfout=\pdfoutB \else
 \let\pdfout=\pdfoutA \fi\fi\fi\fi\fi
 \pdf@ut \@@outline{#1}{#2}{#3}{#4}{#5}\fi\fi}

\def\fourdigits#1{\ifnum#1<0 \errmessage{min is 0}\else
            \ifnum#1>9999 \errmessage{max is 9999}\else
 \ifnum#1<1000 0\fi \ifnum#1<100 0\fi \ifnum#1<10 0\fi\fi\fi \number#1}
\ifx\secid\undefined \let\secid\empty\fi

\ifx\doextrasave\undefined \let\doextrasave=\relax \fi
\ifx\doextrapdf\undefined \let\doextrapdf=\relax \fi

\def\save#1{\begingroup
 \def~{\string~}\def\\{\string\\}\def\S{\string\S}\stringaccents
 \def\&{\string\&}\def\%{\string\%}\def\${\string\$}\def\#{\string\#}%
 \deactivatehigh \utfon\out{utf}\let^^e2=\@eii \doextrasave
 \edef\next{\write\auxf{#1\string{\fourdigits\d@stno\string}%
 \string{\secid\string}\string{\noexpand\folio\string}}}\next\endgroup}

\newwrite\auxf \newwrite\tocf \newwrite\ndxf

\def\files{\begingroup
 \def~{\string~}\def\\{\string\\}\def\-{\string\-}\def\S{\string\S}\stringaccents
 \def\&{\string\&}\def\%{\string\%}\def\${\string\$}\def\#{\string\#}%
 \deactivatehigh \utfon\out{utf}\let^^e2=\@eii \doextrasave
 \def\ftoc##1##2##3##4##5{\ifnum##1<9\pdft@toc{##1}\fi
  \immediate\write\tocf{\string\tocline
   \string{##1\string}\string{##2\string}%
   \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\fndx##1##2##3##4##5{\immediate\write\ndxf{\string\ndxline
  \string{##1\string}\string{##2\string}%
  \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\flbl##1##2##3##4##5{\setbox0=\hbox{\csname ^^03##1\endcsname}%
  \ifdim\wd0=0pt
   \expandafter\gdef\csname ^^02##1\endcsname{##2}% replacement
   \expandafter\gdef\csname ^^03##1\endcsname{##3}% \d@stno
   \expandafter\gdef\csname ^^04##1\endcsname{##4}% \secid
   \expandafter\gdef\csname ^^05##1\endcsname{##5}% \folio
  \else\errmessage{label ##1 redefined}\fi}
 \ifauxf
  \immediate\openout\tocf=auxiliar.toc
  \immediate\openout\ndxf=auxiliar.ind
  \input auxiliar.aux
  \immediate\closeout\tocf \immediate\closeout\ndxf
  \out{pdf}\def\\{ }\def\-{}\doextrapdf
  \pdft@toc0 \catcode`\(=13 \catcode`\)=13
  \ifcase\pdfoutput
   \ifx\dvips\undefined \let\@@outline=\dvipdf@outline
   \else \let\@@outline=\dvips@outline \fi
  \else \let\@@outline=\pdf@outline \fi
  \let\tocline=\@outline
  \input auxiliar.toc
 \fi
 \endgroup
 \openout\auxf=auxiliar.aux
 \def\ref{\r@f^^02}\def\refsc{\r@f^^04}\def\refpg{\r@f^^05}\def\refx{\r@fx}%
 \def\toc##1##2{\save{\string\ftoc\string{##1\string}\string{##2\string}}}%
 \def\lbl##1##2{\save{\string\flbl\string{##1\string}\string{##2\string}}}%
 \def\ndx##1##2{\save{\string\fndx\string{##1\string}\string{##2\string}}}%
}
% Note that \vbox{}someword or someword\vbox{} does not hyphenate someword.

\def\stringaccents{\def\'{\string\'}\def\~{\string\~}\def\"{\string\"}%
 \def\^{\string\^}\def\`{\string\`}}

\def\r@f#1#2{{\stringaccents\def\&{\string\&}\out{utf}\let^^e2=\@eii
  \xdef\n@@{\string"#2\string" }\xdef\@@n{\csname ^^03#2\endcsname}%
  \expandafter\global\expandafter\let\expandafter\@n@\csname #1#2\endcsname}%
 \setbox0=\hbox{\@n@}\ifdim\wd0=0pt ?\ifauxf\errmessage{label \n@@ undefined}\fi
  \else\goto{\@n@}{\@@n}\fi}

\def\r@fx#1#2{{\stringaccents\def\&{\string\&}\out{utf}\let^^e2=\@eii
  \xdef\n@@{\string"#2\string" }\xdef\@@n{\csname ^^03#2\endcsname}}%
 \setbox0=\hbox{\@@n}\ifdim\wd0=0pt ?\ifauxf\errmessage{label \n@@ undefined}\fi
  \else\goto{#1}{\@@n}\fi}

\def\label#1#2{\dest\lbl{#1}{#2}}
\def\index#1#2{\dest\ndx{#1}{#2}}

\catcode`\@=12


==> utf.tex <==
% utf.tex (RMCG20200319)

% To allow utf-8 input.
%
% It is restricted to U+0000 to U+00FF (ISO-8859-1 including ASCII) plus 15 codes in plane U+20xy
% Note that codes U+0000 to U+001F and U+007F to U+009F are control codes,
%    including U+000A (LF) used as line terminator in unix.
% It needs to activate ^^c2, ^^c3, and ^^e2 to work (\utfon to activate, \utfoff to deactivate)
%
% Utf-8 chars starting with bytes ^^c2, ^^c3, and ^^e2 are firstly converted to macro tokens,
%    so, for example ^^c2^^a7 is converted in macro \^^c2^^a7.
%
% It provides for four otputs:
%    1) utf: so macro \^^c2^^a7@utf is defined as {\string^^c2\string^^a7}
%    2) pdf: so macro \^^c2^^a7@pdf is defined as {\string^^a7}
%    3) iso: so macro \^^c2^^a7@iso is defined as {\string^^a7}
%    4) tex: so macro \^^c2^^a7@tex is defined as {\S}
%
% When an out is defined, via the \out{tex} macro, a series of \let operation are performed,
%    as, for example, \let\^^c2^^a7=\^^c2^^a7@tex
% so, if char ^^c2 is active, the input ^^c2^^a7 expands to \S.


\catcode`\@=11

\def\deactivatehigh{\count@=128 \loop \catcode\count@=12
 \ifnum\count@<255 \advance\count@1 \repeat}

\deactivatehigh % just in case

\def\doutfA{%
 \do^^80^^c0\do^^81^^c1\do^^82^^c2\do^^83^^c3\do^^84^^c4\do^^85^^c5\do^^86^^c6\do^^87^^c7%
 \do^^88^^c8\do^^89^^c9\do^^8a^^ca\do^^8b^^cb\do^^8c^^cc\do^^8d^^cd\do^^8e^^ce\do^^8f^^cf%
 \do^^90^^d0\do^^91^^d1\do^^92^^d2\do^^93^^d3\do^^94^^d4\do^^95^^d5\do^^96^^d6\do^^97^^d7%
 \do^^98^^d8\do^^99^^d9\do^^9a^^da\do^^9b^^db\do^^9c^^dc\do^^9d^^dd\do^^9e^^de\do^^9f^^df%
 \do^^a0^^e0\do^^a1^^e1\do^^a2^^e2\do^^a3^^e3\do^^a4^^e4\do^^a5^^e5\do^^a6^^e6\do^^a7^^e7%
 \do^^a8^^e8\do^^a9^^e9\do^^aa^^ea\do^^ab^^eb\do^^ac^^ec\do^^ad^^ed\do^^ae^^ee\do^^af^^ef%
 \do^^b0^^f0\do^^b1^^f1\do^^b2^^f2\do^^b3^^f3\do^^b4^^f4\do^^b5^^f5\do^^b6^^f6\do^^b7^^f7%
 \do^^b8^^f8\do^^b9^^f9\do^^ba^^fa\do^^bb^^fb\do^^bc^^fc\do^^bd^^fd\do^^be^^fe\do^^bf^^ff%
}

% \def\^^c2^^xy@utf{^^c2^^xy} where x = 8-b, y = 0-f
\def\do#1#2{\expandafter\def
 \csname\string^^c2\string#1@utf\endcsname{\string^^c2\string#1}}\doutfA
% \def\^^c3^^xy@utf{^^c3^^xy}
\def\do#1#2{\expandafter\def
 \csname\string^^c3\string#1@utf\endcsname{\string^^c3\string#1}}\doutfA
% \def\^^c2^^xy@pdf{^^xy}
\def\do#1#2{\expandafter\def
 \csname\string^^c2\string#1@pdf\endcsname{\string#1}}\doutfA
% \def\^^c3^^xy@pdf{^^(xy+64}}
\def\do#1#2{\expandafter\def
 \csname\string^^c3\string#1@pdf\endcsname{\string#2}}\doutfA
% \def\^^c3^^xy@iso{^^(xy+64}}
\def\do#1#2{\expandafter\def
 \csname\string^^c2\string#1@iso\endcsname{\string#1}}\doutfA
% \def\^^c3^^xy@pdf{^^(xy+64}}
\def\do#1#2{\expandafter\def
 \csname\string^^c3\string#1@iso\endcsname{\string#2}}\doutfA

\def\tura#1{{\edef\scf@{\the\scriptfont\fam}%
 \ifdim\fontdimen6\scf@=0pt\else\scf@\fi $^{\hbox{\b{#1}}}$}}

% Default case for ^^c2 codes not defiined in plain TeX
\def\do#1#2{\expandafter\def
 \csname\string^^c2\string#1@tex\endcsname{\string#1}}\doutfA

\def\dotexA{%
 \do^^c3^^80{\`A}\do^^c3^^a0{\`a}%
 \do^^c3^^81{\'A}\do^^c3^^a1{\'a}%
 \do^^c3^^82{\^A}\do^^c3^^a2{\^a}%
 \do^^c3^^83{\~A}\do^^c3^^a3{\~a}%
 \do^^c3^^84{\"A}\do^^c3^^a4{\"a}%
 \do^^c3^^85{\AA}\do^^c3^^a5{\aa}%
 \do^^c3^^86{\AE}\do^^c3^^a6{\ae}%
 \do^^c3^^87{\c C}\do^^c3^^a7{\c c}%
 \do^^c3^^88{\`E}\do^^c3^^a8{\`e}%
 \do^^c3^^89{\'E}\do^^c3^^a9{\'e}%
 \do^^c3^^8a{\^E}\do^^c3^^aa{\^e}%
 \do^^c3^^8b{\"E}\do^^c3^^ab{\"e}%
 \do^^c3^^8c{\`I}\do^^c3^^ac{\`\i}%
 \do^^c3^^8d{\'I}\do^^c3^^ad{\'\i}%
 \do^^c3^^8e{\^I}\do^^c3^^ae{\^\i}%
 \do^^c3^^8f{\"I}\do^^c3^^af{\"\i}%
 \do^^c3^^90{D}\do^^c3^^b0{d}% No eth in plain \TeX
 \do^^c3^^91{\~N}\do^^c3^^b1{\~n}%
 \do^^c3^^92{\`O}\do^^c3^^b2{\`o}%
 \do^^c3^^93{\'O}\do^^c3^^b3{\'o}%
 \do^^c3^^94{\^O}\do^^c3^^b4{\^o}%
 \do^^c3^^95{\~O}\do^^c3^^b5{\~o}%
 \do^^c3^^96{\"O}\do^^c3^^b6{\"o}%
 \do^^c3^^97{\times}\do^^c3^^b7{\div}% only in maths
 \do^^c3^^98{\O}\do^^c3^^b8{\o}%
 \do^^c3^^99{\`U}\do^^c3^^b9{\`u}%
 \do^^c3^^9a{\'U}\do^^c3^^ba{\'u}%
 \do^^c3^^9b{\^U}\do^^c3^^bb{\^u}%
 \do^^c3^^9c{\"U}\do^^c3^^bc{\"u}%
 \do^^c3^^9d{\'Y}\do^^c3^^bd{\'y}
 \do^^c3^^9e{P}\do^^c3^^be{p}% No thorn in plain \TeX
 \do^^c3^^9f{\ss}\do^^c3^^bf{\"y}%
 \do^^c2^^a1{!`}\do^^c2^^bf{?`}%
 \do^^c2^^aa{\tura a}\do^^c2^^ba{\tura o}%
 \do^^c2^^a9{\copyright}\do^^c2^^b0{$^\circ$}%
 \do^^c2^^a7{\S}\do^^c2^^b6{\P}%
 \do^^c2^^ab{``}\do^^c2^^bb{''}% No guillomets in plain \TeX
}

% \def\^^c2^^xy@tex{\TeX\ code}
\def\do#1#2#3{\expandafter\def
 \csname\string#1\string#2@tex\endcsname{#3}}\dotexA

\def\doutfB{% list of 3 byte codes accepted
 \do^^e2^^80^^92% figure dash U+2012
 \do^^e2^^80^^93% en dash
 \do^^e2^^80^^94% em dash
 \do^^e2^^80^^98% left single quotation mark
 \do^^e2^^80^^99% right single quotation mark
 \do^^e2^^80^^9a% single low-9 quotation mark
 \do^^e2^^80^^9c% left double quotation mark
 \do^^e2^^80^^9d% right double quotation mark
 \do^^e2^^80^^9e% double low-9 quotation mark
 \do^^e2^^80^^a0% dagger U+2020
 \do^^e2^^80^^a1% double dagger
 \do^^e2^^80^^a6% horizontal ellipsis
 \do^^e2^^80^^b0% per mille sign U+2030
 \do^^e2^^80^^b9% single left-pointing angle quotation mark
 \do^^e2^^80^^ba% single right-pointing angle quotation mark
 \do^^e2^^82^^ac% euro sign U+20AC
}

%\def\^^e2^^8a^^bc@utf{^^e2^^8a^^bc}
\def\do#1#2#3{\expandafter\def
 \csname\string#1\string#2\string#3@utf\endcsname{\string#1\string#2\string#3}}\doutfB

\def\dopdfB{% pdf 80/9f -> utf-8 e2-80-xy
 \do^^81^^a0\do^^82^^a1\do^^83^^a6\do^^84^^94\do^^85^^93\do^^85^^92% † ‡ … — – –
 \do^^88^^b9\do^^89^^ba\do^^8b^^b0\do^^8c^^9e\do^^8d^^9c\do^^8e^^9d\do^^8f^^98% ‹ › ‰ „ “ ” ‘
 \do^^90^^99\do^^91^^9a% ’ ‚
}

%\def\^^e2^^80^^xy@pdf{^^ab}
\def\do#1#2{\expandafter\def
 \csname\string^^e2\string^^80\string#2@pdf\endcsname{\string#1}}\dopdfB

\def\doisoB{% iso 80/9f -> utf-8 e2-80-xy
 \do^^82^^9a\do^^84^^9e\do^^85^^a6\do^^86^^a0\do^^87^^a1% ‚ „ … † ‡
 \do^^8b^^b9% ‰ ‹
 \do^^91^^98\do^^92^^99\do^^93^^9c\do^^94^^9d\do^^96^^92\do^^96^^93\do^^97^^94% ‘ ’ “ ” – – —
 \do^^9b^^ba% ›
}

%\def\^^e2^^80^^xy@iso{^^ab}
\def\do#1#2{\expandafter\def
 \csname\string^^e2\string^^80\string#2@iso\endcsname{\string#1}}\doisoB

\def\dotexB{% utf-8 e2-80-xy -> \TeX
 \do^^92{--}\do^^93{--}\do^^94{---}%
 \do^^98{`}\do^^99{'}\do^^9a{,}\do^^9c{``}\do^^9d{''}\do^^9e{,\kern-1pt,}%
 \do^^a0{\dag}\do^^a1{\ddag}%
 \do^^a6{\dots}%
 \do^^b0{\%\%}\do^^b9{`}\do^^ba{'}%
}

% \def\^^e2^^80^^xy@tex{\TeX\ code}
\def\do#1#2{\expandafter\def
 \csname\string^^e2\string^^80\string#1@tex\endcsname{#2}}\dotexB

% utf-8 other chars

% Euro
\expandafter\def\csname\string^^e2\string^^82\string^^ac@utf\endcsname{\string^^e2\string^^82\string^^ac}
\expandafter\def\csname\string^^e2\string^^82\string^^ac@pdf\endcsname{\string^^a0}
\expandafter\def\csname\string^^e2\string^^82\string^^ac@iso\endcsname{\string^^01}
\def\euro{EUR}% If the symbol is not available, this is its official code
\expandafter\def\csname\string^^e2\string^^82\string^^ac@tex\endcsname{\euro}

% \def\out#1{\let<name>=\<name>@#1}
\def\out#1{\outA@{#1}\csname outB@#1\endcsname}

\def\outA@#1{%
 \def\do##1##2{\expandafter\let\expandafter\next\csname\string^^c2\string##1@#1\endcsname
  \expandafter\let\csname\string^^c2\string##1\endcsname=\next}\doutfA
 \def\do##1##2{\expandafter\let\expandafter\next\csname\string^^c3\string##1@#1\endcsname
  \expandafter\let\csname\string^^c3\string##1\endcsname=\next}\doutfA
}

\def\outB@utf{%
 \def\do##1##2##3{\expandafter\let\expandafter\next
  \csname\string##1\string##2\string##3@utf\endcsname
  \expandafter\let\csname\string##1\string##2\string##3\endcsname=\next}\doutfB
}

\def\outB@pdf{\def\do##1##2{\expandafter\let\expandafter\next
  \csname\string^^e2\string^^80\string##2@pdf\endcsname
 \expandafter\let\csname\string^^e2\string^^80\string##2\endcsname=\next}\dopdfB
 % euro
 \expandafter\let\expandafter\next\csname\string^^e2\string^^82\string^^ac@tex\endcsname
 \expandafter\let\csname\string^^e2\string^^82\string^^ac\endcsname\next
}

\def\outB@iso{\def\do##1##2{\expandafter\let\expandafter\next
  \csname\string^^e2\string^^80\string##2@iso\endcsname
 \expandafter\let\csname\string^^e2\string^^80\string##2\endcsname=\next}\doisoB
 % euro
 \expandafter\let\expandafter\next\csname\string^^e2\string^^82\string^^ac@iso\endcsname
 \expandafter\let\csname\string^^e2\string^^82\string^^ac\endcsname\next
}

\def\outB@tex{\def\do##1##2{\expandafter\let\expandafter\next
  \csname\string^^e2\string^^80\string##1@tex\endcsname
 \expandafter\let\csname\string^^e2\string^^80\string##1\endcsname=\next}\dotexB
 % euro
 \expandafter\let\expandafter\next\csname\string^^e2\string^^82\string^^ac@tex\endcsname
 \expandafter\let\csname\string^^e2\string^^82\string^^ac\endcsname\next
}

\def\utfon{\catcode`\^^c2=13 \catcode`\^^c3=13 \catcode`\^^e2=13 \relax}
\def\utfoff{\catcode`\^^c2=12 \catcode`\^^c3=12 \catcode`\^^e2=12 \relax}

\utfon

\def^^c2#1{\csname\string^^c2\string#1\endcsname}
\def^^c3#1{\csname\string^^c3\string#1\endcsname}
\newhelp\utfhelp{Only a few UTF-8 codes beginning with 0xE2 are implemented.}
\def^^e2#1#2{\expandafter\let\expandafter\next\csname\string^^e2\string#1\string#2\endcsname
 \ifx\next\relax \errhelp=\utfhelp
 \errmessage{UTF-8 char \string^^e2\string#1\string#2 undefined}\fi\next}
\def\@eii#1#2{\csname\string^^e2\string#1\string#2\endcsname}

\catcode`\@=12

\endinput

